Systems for Memory Disaggregation: Challenges & Opportunities

Memory disaggregation addresses memory imbalance in a cluster by decoupling CPU and memory allocations of applications while also increasing the effective memory capacity for (memory-intensive) applications beyond the local memory limit imposed by traditional fixed-capacity servers. As the network speeds in the tightly-knit environments like modern datacenters inch closer to the DRAM speeds, there has been a recent proliferation of work in this space ranging from software solutions that pool memory of traditional servers for the shared use of the cluster to systems targeting the memory disaggregation in the hardware. In this report, we look at some of these recent memory disaggregation systems and study the important factors that guide their design, such as the interface through which the memory is exposed to the application, their runtime design and relevant optimizations to retain the near-native application performance, various approaches they employ in managing cluster memory to maximize utilization, etc. and we analyze the associated trade-offs. We conclude with a discussion on some open questions and potential future directions that can render disaggregation more amenable for adoption.

==> background.tex <==
\section{Background}
\label{sec:background}

% \vspace{5pt}
% \noindent \uline{Historical work.}
% Very early work on improving cluster memory 
% utilization ~\cite{gms,cashmere,treadmarks,dsm1} 
% sticked to traditional server architectures and focused on 
% software-based memory pooling across the cluster and exposing it 
% to applications in (mainly) two different flavors. 
% Distributed shared memory (DSM) systems~\cite{treadmarks,dsm1} 
% provide a global shared address space for writing distributed 
% applications, where the address space is globally accessible 
% from all the servers. These systems can then transparently 
% back subsets of address space (at different granularity) with 
% physical memory from different servers across the cluster, and 
% therefore have the flexibility of optimizing cluster memory 
% utilization. Other systems like GMS~\cite{gms, cashmere} just 
% focus on extending the address space of individual applications 
% without any notion of sharing across servers (i.e., their memory 
% consistency model stops with cache coherence protocols on a single 
% server). These systems merely back or complement local DRAM with 
% unutilized memory from other servers using the paging mechanisms 
% in the operating system, usually by providing remote memory as 
% another block device to swap to. DSM systems 
% provide shared memory (along with some consistency model) which 
% makes distributed programming easier but they may require 
% applications be rewritten using their memory model. Conversely, 
% remote paging systems aim to be more backwards-compatible and 
% leave the complexity of building distributed applications 
% (if needed) to the higher layers. These early systems however 
% hasn't seen adoption (perhaps?) because remote memory latencies 
% were still far higher for tenable application performance. 
% (DSM though had even more challenges due to overheads in 
% ensuring consistency that get amplified with slow networks).
% \vspace{5pt}
% \noindent \uline{Recent proliferation in this space.}
As the remote access latencies come closer to native 
DRAM latencies (which, on the contrary, 
are nearing saturation~\cite{Aguilera2017}),
writing applications with such accesses 
in the critical path is looking feasible, 
performance-wise~\cite{netdisagg}. 
Consequently, there has been a lot of RDMA-inspired remote 
memory system building in recent years, including a renewal in
DSM~\cite{farm, gam,dspm,ltdsm} and Remote 
paging~\cite{Lim2012,bladedisagg1,infiniswap,zswap,fastswap,leap} 
systems. While the remote paging systems provide native virtual memory 
interface (i.e., memory access through load/store ops on cached 
local pages from remote memory) to applications, 
other new interfaces for remote memory were proposed that 
sacrifice application transparency in favor of performance 
due to either the simplicity of 
implementation~\cite{remregions,literdma} (light-weight runtime 
means less performance overhead in the critical access path) or 
benefits from application hints~\cite{aifm}; 
conversely, these interfaces require app modifications but
enable applications to distinguish between local and remote 
memory accesses and be smart about it e.g., use far-memory 
aware implementations~\cite{Aguilera2019,semeru}.

Most systems for disaggregated memory target clusters with 
traditional (commodity) servers where memory is collocated 
with processors and there is no special hardware support.
Traditional hardware cannot access remote memory directly 
and hence usual solutions has to proxy it  
through local memory by caching remote data and resorting to 
software to fetch remote data on a cache miss. To avoid 
this overhead, some systems introduce special hardware 
like a remote memory controller~\cite{sonuma} or a 
cache-coherent FPGA~\cite{kona} to plug into 
the local cache hierarchy and handle remote accesses through 
the hardware. And finally, as an alternative to traditional 
server model, there were proposals for new 
hardware architectures where memory is decoupled and pooled
at a hardware-level, and some systems targeting such 
disaggregation~\cite{sonuma,bladedisagg1,legoos} as well. 
In this report, we will look at many of these systems to 
provide an informed view of disaggregated system design.


==> conclusion.tex <==

\section{CONCLUSION}
\label{sec:conclusion}
In this report, we look at various aspects in  
the design of a disaggregated memory system
guided by recent work in this space. We then 
discuss some untackled challenges and future 
opportunities for further improving such systems. 


==> future.tex <==
FUTURE RESEARCH QUESTIONS FOR YOURSELF
======================================
1. Extending fast swap on how many jobs can 
co-exist decently on a particular compute node 
oversubscribing cache space for local memory?
It depends on locality patterns of the apps,
we find a balanced mixture of apps that can 
do well with fixed amount of local memory
as cache.

2. A kernel-based interface that allows for 
application-runtime co-design. Providing perf 
benefits of userspace runtimes while generality 
and sharing benefits of kernel-based 
implementation. but what's lacking in 
remote regions?

3. Propose a proper hardware architecture for
disaggregation. What's the right amount of 
local memory? Why does it have to be small/big?
It is supposedly small because it's not counting 
towards app memory and hence extra cost. 
The other side of argument is DRAM is cheap now,
so why not; disaggregation is more to overcome 
dram limits on a single server than to save 
memory. what's right here?  




==> related.tex <==
\section{RELATED WORK}
\label{sec:relatedwork}
Systems we looked at in this report?

